Out-of-Distribution Detection by Leveraging Between-Layer Transformation Smoothness

Effective out-of-distribution (OOD) detection is crucial for reliable machine learning models, yet most current methods are limited in practical use due to requirements like access to training data or intervention in training. We present a novel method for detecting OOD data in Transformers based on transformation smoothness between intermediate layers of a network (BLOOD), which is applicable to pre-trained models without access to training data. BLOOD utilizes the tendency of between-layer representation transformations of in-distribution (ID) data to be smoother than the corresponding transformations of OOD data, a property that we also demonstrate empirically. We evaluate BLOOD on several text classification tasks with Transformer networks and demonstrate that it outperforms methods with comparable resource requirements. Our analysis also suggests that when learning simpler tasks, OOD data transformations maintain their original sharpness, whereas sharpness increases with more complex tasks.

==> sections/5-discussion.tex <==
\section{Discussion}

\jan{ovdje stao 2023-09-27}
\fran{I suggest we remove this section.}

%\paragraph{Minimal prerequisites}
%In this work, we presented the idea of OOD detection methods with minimal prerequisites, which are methods that do not require any changes in the standard training procedure of DNNs or the availability of training data during evaluation. We suspect this property could have importance in the real world applications when working with the model that was trained by the third party. We experiment with different baselines we categorized as having minimal prerequisites: MSP, ENT, MC, and GRAD. Even though Monte-Carlo dropout requires that the model's architecture implements dropout \citep{srivastava2014dropout}, dropout is so widely accepted that it has become standard for most popular architectures to implement \citep{liu2019roberta,tan2019efficientnet,clark2020electra,dosovitskiy2021image}, and thus we do not consider it a limiting prerequisite. However, there is another scenario with even less prerequisites than what we call minimal prerequisites in this work. It is looking at the model as a black-box with access only to the inputs and their respective outputs, e.g., model that is embedded in some application. From the utilized baselines, only MSP and ENT fulfill the black-box prerequisites.

\textbf{Our method's assumptions.}~
We introduced the novel approach to tackle the OOD detection task. It relies on the assumption that representations of ID data are transformed differently between layers of DNN than the representations of the OOD data.
Since our approach tracks the change in representations of the model, it requires models to create intermediate representations while encoding data, and thus it is not suitable for shallow models.
In principle, it does not require the models to have a probabilistic output, it only requires the model to have intermediate layers. So, unlike probabilistic methods such as MSP, ENT, and MC, our method can be coupled with the DNN regression model.

\textbf{Limitations.}~
Our method has no theoretical grounding (yet), unlike, for example, Monte-Carlo Dropout methods. It is based on our intuition and encouraging empirical results.
Furthermore, our method is not probabilistic and, as such, can not be calibrated. It can only be used to compare how uncertain the model is about different instances.
It also has different scales for different hypotheses, so it can not be used to compare the uncertainties of different hypotheses.


==> sections/B-proof-long.tex <==
\section{Proof of lemma 1}
\label{sec:appendix:proof}

\begin{replemma}{thr:estimate}
   Let $\mJ(\vx) \in \R^{m \times n}$ be a Jacobian matrix, and let $\rvv \in \R^n$ and $\rvw \in \R^m$ be random vectors whose elements are independent random variables with zero mean and unit variance. Then, $\E[(\rvw^{\intercal}\mJ(\vx)\rvv)^2] = \| \mJ(\vx) \|_F^2$.
\end{replemma}
%
\begin{proof}
    Firstly, we expand the vector-Jacobian-vector product of a Jacobian matrix $\mJ = \frac{\partial \rvy}{\partial \rvx}$:
    \begin{align*}
        (\rvw^{\intercal}\mJ\rvv)^2 &= \left(\sum_{i} \evw_i \sum_{j} \evv_j \frac{\partial \evy_j}{\partial \evx_i} \right)^2\\
        &= \left(\sum_{i} \sum_{j} \evw_i \evv_j \frac{\partial \evy_j}{\partial \evx_i} \right)^2.
    \end{align*}
%
    Expansion of the square of the outer sum:
    \begin{align*}
        &= \underbrace{\sum_i \left( \sum_j \evw_i \evv_j \frac{\partial \evy_j}{\partial \evx_i} \right)^2}_{\textcircled{x}}
        + \underbrace{2 \sum_i \sum_{k<j} \left( \sum_j \evw_i \evv_j \frac{\partial \evy_j}{\partial \evx_i} \right) \left( \sum_j \evw_k \evv_j \frac{\partial \evy_j}{\partial \evx_k} \right)}_{\textcircled{c}}.
    \end{align*}
%
    Expansion of the square of the inner sum:
    \begin{align*}
        \textcircled{x} &= \sum_i \left( \sum_j \evw_i \evv_j \frac{\partial \evy_j}{\partial \evx_i} \right)^2\\
        &= \sum_i \left[ \sum_j \left( \evw_i\evv_j \frac{\partial \evy_j}{\partial \evx_i} \right)^2
        + 2 \sum_i \sum_{k<j} \left( \evw_i \evv_j \frac{\partial \evy_j}{\partial \evx_i} \right) \left( \evw_i \evv_k \frac{\partial \evy_k}{\partial \evx_i} \right) \right]\\
        &= \underbrace{\sum_i \sum_j \left( \evw_i \evv_j  \frac{\partial \evy_j}{\partial \evx_i}\right)^2}_{\textcircled{a}}
        + \underbrace{2 \sum_i \sum_j \sum_{k<j} \left( \evw_i \evv_j  \frac{\partial \evy_j}{\partial \evx_i} \right) \left( \evw_i \evv_k  \frac{\partial \evy_k}{\partial \evx_i} \right)}_{\textcircled{b}}.
    \end{align*}
%
    So the vector-Jacobian-vector product can be expanded as a sum:
    \begin{align}
        \left( \rvw^{\intercal}\mJ\rvv \right)^2 &= \textcircled{a} + \textcircled{b} + \textcircled{c}. \label{eq:sum-formulation}
    \end{align}
%
    \begin{lemma}
        \label{thr:sqr}
        The expected value of a random variable $\ra$ squared with $\E[\ra]=0$ and $\Var[\ra]=1$ is $\E[\ra^2]=1$.
    \end{lemma}
%
    \begin{proof}
        $\Var[\ra] = \E[\ra^2] - \E[\ra]^2$. After rearranging and substituting $\E[\ra] = 0$ and $\Var[\ra] = 1$, we get $\E[\ra^2] = \E[\ra]^2 + \Var[\ra] = 0 + 1 = 1$.
    \end{proof}
%
    \begin{lemma}
        \label{thr:mul}
        The expected value of a product of two independently and identically distributed random variables $\ra$ and $\rb$ is $\E[\ra \rb]$ if either $\E[\ra] = 0$ or $\E[\rb] = 0$.
    \end{lemma}
%
    \begin{proof}
        For two independently and identically distributed random variables $\ra$ and $\rb$ the expected value $\E[\ra \rb] = \E[\ra]\E[\rb] = 0$ when $\E[\ra]$ or $\E[\rb]$ is $0$.
    \end{proof}
%
    For deriving an expected value of the vector-Jacobian-vector product we will calculate the expected value of its sum formulation from \Cref{eq:sum-formulation} with the help of Lemmas \ref{thr:sqr} and \ref{thr:mul}:
%
    \begin{align}
        \E[(\rvw^{\intercal}\mJ\rvv)^2] &= \E[\textcircled{a} + \textcircled{b} + \textcircled{c}]\\
        &= \E[\textcircled{a}] + \E[\textcircled{b}] + \E[\textcircled{c}].\label{eq:sum-expected}
    \end{align}
%
    Now we need to calculate the expected values of $\textcircled{a}$, $\textcircled{b}$, and $\textcircled{c}$:
%
    \begin{align*}
        \E[\textcircled{a}] &= \E\left[ \sum_i \sum_j \left( \evw_i \evv_j \frac{\partial \evy_j}{\partial \evx_i} \right)^2 \right],\\
        &= \E\left[\sum_i \sum_j \evw_i^2 \evv_j^2 \left( \frac{\partial \evy_j}{\partial \evx_i} \right)^2 \right]\\
        &= \sum_i \sum_j \underbrace{\E[\evw_i^2]}_{1} \underbrace{\E[\evv_j^2]}_{1} \left[\left( \frac{\partial \evy_j}{\partial \evx_i} \right)^2\right]\\
        &= \sum_i \sum_j \left( \frac{\partial \evy_j}{\partial \evx_i} \right)^2,
    \end{align*}
%
    \begin{align*}
         \E[\textcircled{b}] &= \E\left[ 2 \sum_i \sum_j \sum_{k<j} \left( \evw_i \evv_j  \frac{\partial \evy_j}{\partial \evx_i} \right) \left( \evw_i \evv_k  \frac{\partial \evy_k}{\partial \evx_i} \right) \right]\\
         &= 2 \sum_i \sum_j \sum_{k<j} \E \left[ \left( \evw_i \evv_j  \frac{\partial \evy_j}{\partial \evx_i} \right) \left( \evw_i \evv_k  \frac{\partial \evy_k}{\partial \evx_i} \right) \right]\\
         &= 2 \sum_i \sum_j \sum_{k<j} \E \left[ \evw_i^2 \evv_j \evv_k \frac{\partial \evy_j}{\partial \evx_i} \frac{\partial \evy_k}{\partial \evx_i} \right]\\
         &= 2 \sum_i \sum_j \sum_{k<j} \underbrace{\E[\evw_i^2]}_1 \underbrace{\E[\evv_j]}_0 \underbrace{\E[\evv_k]}_0 \frac{\partial \evy_j}{\partial \evx_i} \frac{\partial \evy_k}{\partial \evx_i}\\
         &= 0,
    \end{align*}
%
    \begin{align*}
        \E[\textcircled{c}] &= \E \left[ 2 \sum_i \sum_{k<j} \left( \sum_j \evw_i \evv_j \frac{\partial \evy_j}{\partial \evx_i} \right) \left( \sum_j \evw_k \evv_j \frac{\partial \evy_j}{\partial \evx_k} \right) \right]\\
        &= 2 \sum_i \sum_{i<k} \E \left[ \left( \sum_j \evw_i \evv_j \frac{\partial \evy_j}{\partial \evx_i} \right) \left( \sum_j \evw_k \evv_j \frac{\partial \evy_j}{\partial \evx_k} \right) \right],
    \end{align*}
%
    since the product $\left( \sum_j \evw_i \evv_j \frac{\partial \evy_j}{\partial \evx_i} \right) \left( \sum_j \evw_k \evv_j \frac{\partial \evy_j}{\partial \evx_k} \right)$ contains two sums with the same index $j$ we substitute the index $j$ of the left sum with $n$, and the index of the right sum with $m$:
%
    \begin{align*}
        &= 2 \sum_i \sum_{i<k} \E \left[ \left( \sum_n \evw_i \evv_n \frac{\partial \evy_n}{\partial \evx_i} \right) \left( \sum_m \evw_k \evv_m \frac{\partial \evy_m}{\partial \evx_k} \right) \right]\\
        &= 2 \sum_i \sum_{i<k} \E \left[ \sum_n \sum_m \evw_i \evw_k \evv_n \evv_m \frac{\partial \evy_n}{\partial \evx_i} \frac{\partial \evy_m}{\partial \evx_k} \right]\\
        &= 2 \sum_i \sum_{i<k} \sum_n \sum_m \underbrace{\E[\evw_i]}_0 \underbrace{\E[\evw_k]}_0 \underbrace{\E[\evv_n \evv_m]}_{\text{$1$ if $n=m$, $0$ otherwise}} \frac{\partial \evy_n}{\partial \evx_i} \frac{\partial \evy_m}{\partial \evx_k}\\
        &= 0.
    \end{align*}
%
    And lastly, we need to substitute the expected values of $\textcircled{a}$, $\textcircled{b}$, and $\textcircled{c}$ back into the \Cref{eq:sum-expected} to get the expected value of the vector-Jacobian-vector product we were after:
%
    \begin{align}
        \E[(\rvw^{\intercal}\mJ\rvv)^2] &= \E[\textcircled{a}] + \E[\textcircled{b}] + \E[\textcircled{c}] = \sum_i \sum_j \left( \frac{\partial \evy_j}{\partial \evx_i} \right)^2 + 0 + 0\\
        &= \sum_i \sum_j \left( \frac{\partial \evy_j}{\partial \evx_i} \right)^2 = ||\mJ||_F^2.
    \end{align}
\end{proof}

\begin{remark}
    Note that even though in this proof we focused on the Jacobian matrix $\mJ$ because of its relevance to our work, the \Cref{thr:estimate} holds for any $m \times n$ matrix $\mM$.
\end{remark}
